DiffRed: Dimensionality Reduction guided by stable rank

In this work, we propose a novel dimensionality reduction technique, DiffRed, which first projects the data matrix, A, along first $k_1$ principal components and the residual matrix $A^{*}$ (left after subtracting its $k_1$-rank approximation) along $k_2$ Gaussian random vectors. We evaluate M1, the distortion of mean-squared pair-wise distance, and Stress, the normalized value of RMS of distortion of the pairwise distances. We rigorously prove that DiffRed achieves a general upper bound of $O\left(\sqrt{\frac{1-p}{k_2}}\right)$ on Stress and $O\left(\frac{(1-p)}{\sqrt{k_2*\rho(A^{*})}}\right)$ on M1 where $p$ is the fraction of variance explained by the first $k_1$ principal components and $\rho(A^{*})$ is the stable rank of $A^{*}$. These bounds are tighter than the currently known results for Random maps. Our extensive experiments on a variety of real-world datasets demonstrate that DiffRed achieves near zero M1 and much lower values of Stress as compared to the well-known dimensionality reduction techniques. In particular, DiffRed can map a 6 million dimensional dataset to 10 dimensions with 54% lower Stress than PCA.

==> figure_files/m1-plot-rmap.tex <==
\begin{figure*}[t]
    \centering
    \captionsetup{font=small}
    \begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/m1-plot-rmap1.png}
    \caption{Dependence of M1 for Random Maps on stable rank described in Corollary \ref{cor:RMapM1Bound}.($d=10$) [\textit{gRS}: geneRNASeq, \textit{R30k}: Reuters30k]}
    \label{fig:m1-plot-rmap1}
\end{subfigure}%
~
\begin{subfigure}[t]{0.5\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/m1-plot-rmap2.png}
    \caption{Variation of M1 with target dimension for Reuters30k}
    \label{fig:m1-plot-rmap2}
\end{subfigure}
\caption{Plots giving insights into the results obtained for Random Map}
\end{figure*}

==> figure_files/stress-plots.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[scale=0.15]{figures/stress_plot_cifar10.png}
    \caption{Cifar10}
    \label{fig:stress-plot-cifar10}
\end{subfigure}%
~
\begin{subfigure}[t]{0.25\textwidth}
    \centering
    \includegraphics[scale=0.15]{figures/stress_plot_hatespeech.png}
    \caption{Hatespeech}
    \label{fig:stress-plot-hatespeech}
\end{subfigure}
\caption{Log-scale plot of stress with target dimension}
\end{figure}

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> tables/div2k_table.tex <==
% \begin{table}[H]
% \captionsetup{font=footnotesize}
% \resizebox{0.5\columnwidth}{!}{%
% \begin{tabular}{|c|ccc|}
% \hline
%                       & \multicolumn{3}{c|}{$\Lambda_S$}                                      \\ \cline{2-4} 
% \multirow{-2}{*}{$d$} & \multicolumn{1}{c|}{DiffRed}       & \multicolumn{1}{c|}{PCA}  & RMap \\ \hline
% 10                    & \multicolumn{1}{c|}{\textbf{0.14}} & \multicolumn{1}{c|}{0.31} & 0.16 \\ \hline
% 20                    & \multicolumn{1}{c|}{\textbf{0.09}} & \multicolumn{1}{c|}{0.26} & 0.11 \\ \hline
% 30                    & \multicolumn{1}{c|}{\textbf{0.07}} & \multicolumn{1}{c|}{0.23} & 0.09 \\ \hline
% {\color[HTML]{FE0000} 40} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} \textbf{0.06}}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 0.21}} & {\color[HTML]{FE0000} 0.08} \\ \hline
% \end{tabular}
% }
% \caption{Comparision of \textit{DiffRed} with PCA and RMap  on Stress ($\Lambda_S$) for DIV2k ($D$=6.6Mn)}
% \label{tab:stress-results-div2k}
% \end{table}




\begin{table}[ht]
\captionsetup{font=scriptsize}
    \begin{subtable}{0.25\textwidth}
        \captionsetup{font=scriptsize}
        \centering
        \resizebox{0.7\textwidth}{!}{%
            \begin{tabular}{|c|ccc|}
                \hline
                                  & \multicolumn{3}{c|}{$\Lambda_S$}                                      \\ \cline{2-4} 
                \multirow{-2}{*}{$d$} & \multicolumn{1}{c|}{DiffRed}       & \multicolumn{1}{c|}{PCA}  & RMap \\ \hline
                10                    & \multicolumn{1}{c|}{\textbf{0.14}} & \multicolumn{1}{c|}{0.31} & 0.16 \\ \hline
                20                    & \multicolumn{1}{c|}{\textbf{0.09}} & \multicolumn{1}{c|}{0.26} & 0.11 \\ \hline
                30                    & \multicolumn{1}{c|}{\textbf{0.07}} & \multicolumn{1}{c|}{0.23} & 0.09 \\ \hline
                {\color[HTML]{FE0000} 40} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} \textbf{0.06}}} & \multicolumn{1}{c|}{{\color[HTML]{FE0000} 0.21}} & {\color[HTML]{FE0000} 0.08} \\ \hline
            \end{tabular}
        }
        \caption{Comparison of \textit{DiffRed} with PCA and RMap  on Stress ($\Lambda_S$) for DIV2k ($D$=6.6Mn)}
        \label{tab:stress-results-div2k}
    \end{subtable}%
    ~
    \begin{subtable}{0.25\textwidth}
     \captionsetup{font=scriptsize}
        \centering
        \resizebox{0.7\textwidth}{!}{%\textbf{}
        \begin{tabular}{|c|ccc|}
            \hline
            \multirow{2}{*}{$d$} & \multicolumn{3}{c|}{$\Lambda_S$}                                      \\ \cline{2-4} 
                                 & \multicolumn{1}{c|}{DiffRed}       & \multicolumn{1}{c|}{PCA}  & RMap \\ \hline
            10                   & \multicolumn{1}{c|}{\textbf{0.10}} & \multicolumn{1}{c|}{0.12} & 0.16 \\ \hline
            20                   & \multicolumn{1}{c|}{\textbf{0.05}} & \multicolumn{1}{c|}{0.08} & 0.11 \\ \hline
            30                   & \multicolumn{1}{c|}{\textbf{0.03}} & \multicolumn{1}{c|}{0.06} & 0.09 \\ \hline
            40                   & \multicolumn{1}{c|}{\textbf{0.02}} & \multicolumn{1}{c|}{0.05} & 0.08 \\ \hline
        \end{tabular}
        }
        \caption{Comparison of \textit{DiffRed} with PCA and RMap  on Stress ($\Lambda_S$) for APTOS 2019 ($D$=509k)}
        \label{tab:stress-results-aptos}
    \end{subtable}
    \caption{Comparison of stress between \textit{DiffRed}, PCA and RMaps on high dimensional datasets}
    \label{tab:stress-results-hdd}
\end{table}




==> tables/preprocessing-tsne-stress.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llll}
\multirow{2}{*}{Dataset} & \multicolumn{3}{l}{Preprocessing to T-SNE} \\
                         & DiffRed       & PCA          & None        \\
Bank                     & 59.66         & 55.61        & 52.44       \\
Hatespeech               & 38.96         & 39.13        & 32.86       \\
FMnist                   & 24.61         & 28.03        & 24.49       \\
Cifar10                  & 17.59         & 22.36        &             \\
geneRNASeq               & 155.36        & 218.94       &             \\
Reuters30k               & 14.31         & 33.68        &            
\end{tabular}
\caption{}
\label{tab:my-table}
\end{table}

==> tables/stress-k1-k2-gene.tex <==
\begin{table}[H]
\centering
\captionsetup{font=scriptsize}
\resizebox{0.35\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{$d$} & \textbf{$k_1$} & \textbf{$k_2$} & \textbf{$\Lambda_{S}$} \\ \hline
10           & 5              & 5              & 0.13                   \\
20           & 8              & 12             & 0.07                   \\
30           & 10             & 20             & 0.05                   \\
40           & 10             & 30             & 0.04                   \\ \hline
\end{tabular}
}
\caption{Stress of geneRNASeq($\rho_A$=1.12)  for different values of $k_1$ and $k_2$.  The table shows experimentally observed optimal values of $k_1$ and $k_2$ for each target dimension.}
\label{tab:stress-k1-k2-gene}
\end{table}

==> tables/stress-k1-k2-reuters.tex <==
\begin{table}[H]
\centering
\captionsetup{font=scriptsize}
\resizebox{0.35\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{$d$} & \textbf{$k_1$} & \textbf{$k_2$} & \textbf{$\Lambda_{S}$} \\ \hline
10           & 0              & 10             & 0.16                   \\
20           & 2              & 18             & 0.11                   \\
30           & 2              & 28             & 0.09                   \\
40           & 4              & 36             & 0.08                   \\ \hline
\end{tabular}
}
\caption{Stress of Reuters30k($\rho_A$=14.50) for different values of $k_1$ and $k_2$. The table shows experimentally observed optimal values of $k_1$ and $k_2$ for each target dimension.}
\label{tab:stress-k1-k2-reuters}
\end{table}
